Robust Perception-Based Navigation using PAC-NMPC with a Learned Value Function

Nonlinear model predictive control (NMPC) is typically restricted to short, finite horizons to limit the computational burden of online optimization. As a result, global planning frameworks are frequently necessary to avoid local minima when using NMPC for navigation in complex environments. By contrast, reinforcement learning (RL) can generate policies that minimize the expected cost over an infinite-horizon and can often avoid local minima, even when operating only on current sensor measurements. However, these learned policies are usually unable to provide performance guarantees (e.g., on collision avoidance), especially when outside of the training distribution. In this paper, we augment Probably Approximately Correct NMPC (PAC-NMPC), a sampling-based stochastic NMPC algorithm capable of providing statistical guarantees of performance and safety, with an approximate perception-based value function trained via RL. We demonstrate in simulation that our algorithm can improve the long-term behavior of PAC-NMPC while outperforming other approaches with regards to safety for both planar car dynamics and more complex, high-dimensional fixed-wing aerial vehicle dynamics. We also demonstrate that, even when our value function is trained in simulation, our algorithm can successfully achieve statistically safe navigation on hardware using a 1/10th scale rally car in cluttered real-world environments using only current sensor information.

==> background.tex <==
\section{Background}

\subsection{PAC-NMPC}
Probably Approximately Correct NMPC (PAC-NMPC) \cite{10250934} is a sampling-based SNMPC method which minimizes an upper confidence bound on the expected cost and probability of constraint violation of a local feedback policy. Consider the stochastic dynamical system, $p(\bx_{t+1}|\bx_{t}, \bu_{t})$, where $\bx_{t}\in\mathbb{R}^{N_x}$ is the state and $\bu_{t}\in\mathbb{R}^{N_u}$ is the control inputs. PAC-NMPC formulates the search for a control policy, $\bu_{t}= \bpi(\bx_t,\bU)$, as a stochastic optimization problem. This is achieved by sampling policy parameters, $\bU$, from a surrogate distribution, $p(\bU|\bnu)$, defined by hyper-parameters $\bnu$. For a discrete-time trajectory sequence $\bX=\{\bx_0,\bu_0, \bx_1,\bu_1 ..., \bu_{N_T-1}, \bx_{N_T} \}$, one can define a non-negative trajectory cost function, $J(\bX) \ge 0$, and a trajectory constraint violation function $C(\bX) \in \{0, 1\}$. During each planning interval, PAC-NMPC iteratively optimizes
\begin{align}
    \bnu^* = \argmin_{\bnu}\min_{\alpha>0} (\mathcal{J}^+_\alpha(\bnu) + \gamma \mathcal{C}^+_\alpha(\bnu)),
\end{align}
where $\mathcal{J}^+_\alpha(\bnu)$ and $\mathcal{C}^+_\alpha(\bnu)$ are PAC bounds on the expectation of $J(\bX)$ and $C(\bX)$ given $p(\bU|\bnu)$. $\gamma > 0$ is a heuristic weighting coefficient. These PAC bounds were derived in \cite{kobilarov2015sample} and guarantee
\begin{align}
    \mathbb{P}\left(\mathbb{E}_{\bX, \bU \sim p(\cdot, \cdot|\bnu)}\left[J(\bX)\right] \leq \mathcal{J}^+_\alpha(\bnu)\right) \geq 1 - \delta, \\
    \mathbb{P}\left(\mathbb{E}_{\bX, \bU \sim p(\cdot, \cdot|\bnu)}\left[C(\bX)\right] \leq \mathcal{C}^+_\alpha(\bnu)\right) \geq 1 - \delta. \label{eq:constraint_pac_bound}
\end{align}
They are not only optimization targets, but also provide probabilistic guarantees of performance and safety. PAC-NMPC can be used with nonlinear dynamics of the general form $\bx_{t+1} \sim p(\cdot|\bx_{t}, \bu_{t})$ as long  as the nominal dynamics used for feedback, $\bff(\bx_t^d,\bu_t^d)$, are differentiable.


\subsection{Actor Critic Reinforcement Learning}
\label{sec:ACRL}
Actor Critic algorithms are policy gradient approaches to solve Markov decision processes (MDP) by simultaneously learning a policy and action-value function \cite{sutton2018reinforcement}. Consider a MDP with states $\bs_t \in \mathbb{R}^{N_s}$, actions $\ba_t \in \mathbb{R}^{N_a}$, transition dynamics $p(\bs_{t+1}|\bs_{t}, \ba_{t})$, and reward function $r(\bs_t, \ba_t)$, where $t$ denotes the time index. The discounted return is defined as the sum of the discounted future rewards of a state-action sequence, $R^{\gamma_d}_t = \sum_{i=t}^\infty\left\{\gamma_d^{i-t}r(\bs_i, \ba_i)\right\}$ where, $\gamma_d \in [0, 1)$ is a discount factor. The action-value function (Q-function), $Q^{\bpi}(\bs_t, \ba_t) = \mathbb{E}\left[R^{\gamma_d}_t \middle| \bs_t, \ba_t\right]$, is the expected discounted return after taking an action $\ba_t$ from state $\bs_t$ and then following policy $\bs_t = \bpi(\ba_t)$. The value function, $V^{\bpi}(\bs_t) = Q^{\bpi}(\bs_t, \bpi(\bs_t))$, is the expected discounted return of following a policy, $\bs_t = \bpi(\ba_t)$, from a given state $\bs_t$. Actor-critic algorithms learn parameters $\bphi$ for an actor policy, $\bpi^{\bphi}(\bs_t)$, and parameters $\bpsi$ for a critic action-value function, $Q^{\bpsi}(\bs_t, \ba_t)$, which estimate the optimal policy $\bpi^*(\bs_t)$ and action-value function $Q^{\bpi^*}(\bs_t, \ba_t)$ where
\begin{align}
\bpi^*(\bs_t) &= \ba_t^* = \argmin_{\ba_t} \mathbb{E}\left[Q^{\bpi^*}(\bs_t, \ba_t)\right], \\
Q^{\bpi^*}(\bs_t, \ba_t^*) &= \mathbb{E}\left[{r(\bs_t, \ba^*_t) + \gamma_d Q^{\bpi^*}(\bs_{t+1}, \ba_{t+1}^*)}\right].
\end{align}

==> introduction.tex <==
\section{Introduction}

Over the past decade, reinforcement learning (RL) has demonstrated impressive control policies that can effectively reason about perception information to perform sophisticated tasks in complex environments \cite{singh2022reinforcement, zhu2021deep, dong2023review}. However, because these RL algorithms require large amounts of data, they are often trained in simulation (e.g., \cite{mirowski2016learning, zhu2017target, long2018towards}). This dependence on simulation and the inability of the RL trained policies to guarantee the satisfaction of general state constraints can frequently lead to degraded, and potentially unsafe, performance when the policy is deployed in the real-world or when it is used in out-of-distribution environments. 

In recent years, nonlinear model predictive control (NMPC) has also served as an effective approach for perception-based robot navigation (e.g., \cite{polevoy2022post, polevoy2022complex, falanga2018pampc, lee2020aggressive, brito2019model, jian2023dynamic}). In some cases, robust and stochastic NMPC (RNMPC and SNMPC respectively) can provide performance guarantees in the presence of uncertainty \cite{lew2021sampling, wu2023robust, yin2023risk, 10250934}. However, NMPC is typically restricted to short, finite horizons to limit the computational burden of online optimization. This often limits controller performance, since the cost accrued over the short horizon is often a poor approximation of the true cost-to-go. For example, in navigation tasks, an inaccurate terminal cost can lead to the system getting caught in local minima or colliding with obstacles, especially when sensor range or field-of-view is limited. Oftentimes, the terminal cost for NMPC is computed using a global planner (e.g., \cite{jian2023dynamic, polevoy2022post, wang2022chase}) with reduced-order models or hand designed heuristics (e.g., \cite{sprinkle2004encoding}), which can lead to sub-optimal performance.

\begin{figure}[]
    \centering
    \includegraphics[trim={0 5 0 20},clip,width=\columnwidth]{images/main_image_updated.png}
    \caption{a) Rally car navigating through obstacle field using NMPC with learned value function and LiDAR. b) Timelapse of rally car navigating through barrels using RL trained actor policy. c) Timelapse of rally car navigating through barrels using PAC-NMPC with learned value function (reaches goal).}
    \vspace{-2em} % TODO: Fix spacing issue, bad practice, find a better solution
    \label{fig:main_img}
\end{figure}

 % \cite{kobilarov2015sample}

In this paper, we augment a sampling-based SNMPC algorithm, PAC-NMPC \cite{10250934}, with an RL-trained perception-informed value function to achieve perception-based navigation with statistical performance guarantees. We first train an actor and critic via reinforcement learning and use Monte Carlo dropout to capture network uncertainty. We then combine the actor and critic to approximate an optimal value function distribution which is sampled by PAC-NMPC, to evaluate final costs and constraints. This affords our approach the long-rage behavior of the RL policy, which minimizes an expected infinite-horizon cost-to-go based on sensor measurements, and the statistical safety guarantees of PAC-NMPC achieved by optimizing sample-complexity bounds \cite{kobilarov2015sample} at run-time. Following the framework established by the survey paper \cite{brunke2022safe}, our method would be classified as Safety Level I. However, the strength of our approach is in the robustness it affords, as well as the formal statistical guarantees of performance it provides at run-time.

Our main contribution is a control algorithm that combines PAC-NMPC and RL to achieve safe perception-based navigation with probabilistic performance guarantees even when the learned value function may be uncertain and approximate. We also present a framework for reducing RL policy training time by using predicted sensor values at runtime to evaluate the cost-to-go at the terminal trajectory state. Finally, we contribute a set of simulation and hardware experiments to evaluate our algorithm and demonstrate safe perception-informed navigation, improved sim-to-real transfer, and robustness to modestly out-of-distribution environments. Our approach is, to the best of our knowledge, the first to combine an RL trained value function (cost-to-go) using high-dimensional perception inputs with NMPC for navigation and obstacle avoidance and the first to quantify and utilizes value function uncertainty to form performance guarantees.

